Artemis: Articulated Neural Pets with Appearance and Motion synthesis

We, humans, are entering into a virtual era and indeed want to bring animals to the virtual world as well for companion. Yet, computer-generated (CGI) furry animals are limited by tedious off-line rendering, let alone interactive motion control. In this paper, we present ARTEMIS, a novel neural modeling and rendering pipeline for generating ARTiculated neural pets with appEarance and Motion synthesIS. Our ARTEMIS enables interactive motion control, real-time animation, and photo-realistic rendering of furry animals. The core of our ARTEMIS is a neural-generated (NGI) animal engine, which adopts an efficient octree-based representation for animal animation and fur rendering. The animation then becomes equivalent to voxel-level deformation based on explicit skeletal warping. We further use a fast octree indexing and efficient volumetric rendering scheme to generate appearance and density features maps. Finally, we propose a novel shading network to generate high-fidelity details of appearance and opacity under novel poses from appearance and density feature maps. For the motion control module in ARTEMIS, we combine state-of-the-art animal motion capture approach with recent neural character control scheme. We introduce an effective optimization scheme to reconstruct the skeletal motion of real animals captured by a multi-view RGB and Vicon camera array. We feed all the captured motion into a neural character control scheme to generate abstract control signals with motion styles. We further integrate ARTEMIS into existing engines that support VR headsets, providing an unprecedented immersive experience where a user can intimately interact with a variety of virtual animals with vivid movements and photo-realistic appearance. We make available our ARTEMIS model and dynamic furry animal dataset at https://haiminluo.github.io/publication/artemis/.

==> overview.tex <==
\section{OVERVIEW}
Humans are entering into the virtual reality era, yet our animal friends have been left behind. To bring animals into the digit world, there are several major problems have yet to be solved. First, we need real-time but high-quality rendering technique to synthesize animal animations with high realism, especially for those fur details. Besides, we lack enough animal motion data to simulate the virtual animals, especially in a controllable manner for intimate interactions.
To address these issues, we introduce a neural framework called ARTEMIS, which consists of two core components: 1) neural animal modeling and rendering and 2) neural motion control and synthesis, as illustrated in Fig.~2. 
Our ARTEMIS system enables interactive motion control, realistic animation, and high quality rendering of furry digital animals, all in real-time, which supports surreal interactions with virtual animals in VR experience.



\paragraph{Neural Animal Modeling and Rendering.}
In this module, we propose a neural-generated (NGI) animal pipeline. It takes the skeletal rig and skinning weights and multi-view RGBA images in representative poses rendered by existing a CGI animal asset as input, and after training enables photo-realistic real-time rendering with appearance, fur and opacity details.
For NGI animal, we build a dynamic neural representation which combines sparse voxel-based octree, explicit skeletal warping, Spherical Harmonics (SHs) and NeRF-like volumetric rendering. 
We design a fast dynamic Octree reconstruction scheme with highly efficient Octree-based feature indexing. 
We further introduce a tailored neural rendering scheme consisting of both a view-dependent volumetric rendering and a 2D neural shading network. 
As a result, our data-driven NGI animal is end-to-end trainable and shares the same skeletal input and rendering output formats as traditional CGI one.
It enables photo-realistic rendering of fur and appearance details, but in a real-time fashion with notably three to four orders of magnitude speed up.


\paragraph{Neural Motion Capture and Synthesis}
This module aims to provide vivid and controllable skeletal motions to previous module so as to enable interactive experience of NGI animals in our ARTEMIS.
Here, we build a hybrid animal motion capture system with multi-view RGB and Vicon cameras to provide a rive movement dataset for our NGI animals.
We propose a robust optimization scheme to reconstruct the corresponding realistic 3D skeletal poses from the multi-modal input for each kind of animal.
Then, we adopt the notable neural character animation approach LMP~~\cite{starke2020local} to generate abstract control signals and  motion styles from these reconstructed skeletal motions, so as to enable a user to controllable guide the move of NGI animals and preview the realistic rendering results in real-time.
We further integrate ARTEMIS into existing consumer-level VR headset platforms for immersive VR experience of NGI animals.
Specifically, we propose a stereo optimization and a hybrid rendering scheme to enhance our neural NGI animal rendering with the classical rasterization of the CGI scenes.
We also capture the skeletal pose of the user to use the user's skeletal motion to guild the abstract control signals of NGI animals.
We provide a variety of VR applications using our ARTEMIS system, which enables the users to intimately interact with various photo-realistic digital animals under vivid movements in virtual space.



